LEO Satellite and RIS: Two Keys to Seamless Indoor and Outdoor Localization

The contemporary landscape of wireless technology underscores the critical role of precise localization services. Traditional global navigation satellite systems (GNSS)-based solutions, however, fall short when it comes to indoor environments, and existing indoor localization techniques such as electromagnetic fingerprinting methods face challenges of additional implementation costs and limited coverage. This article explores an innovative solution that blends low Earth orbit (LEO) satellites with reconfigurable intelligent surfaces (RISs), unlocking its potential for realizing seamless indoor and outdoor localization (SIOL) with global coverage. After a comprehensive review of the distinctive characteristics of LEO satellites and RISs, we showcase their potential for SIOL applications through two case studies on position error bound evaluation. Finally, we discuss system architectures and highlight open challenges in such systems.

==> figures/CN0.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.5, 0.8, 0.5}%
\definecolor{mycolor2}{rgb}{1.0, 0.5, 0.31}%
%
\begin{tikzpicture}
\begin{axis}[%
width=2.821in,
height=1.686in,
at={(0.758in,0.481in)},
scale only axis,
bar shift auto,
xmin=0.514285714285714,
xmax=5.48571428571429,
xtick={1,2,3,4,5},
xlabel style={font=\color{white!15!black},font=\footnotesize},
xticklabel style = {font=\color{white!15!black},font=\footnotesize},
xticklabels={{Starlink},{Kuiper},{GPS},{Galileo},{BeiDou}},
ymin=0,
ymax=55,
ytick={0,10,20,30,40,50},
ylabel near ticks, % Add this line
ylabel style={font=\color{white!15!black},font=\footnotesize},
yticklabel style = {font=\color{white!15!black},font=\footnotesize},
ylabel={$\text{C/N}_\text{0}\text{ (dB-Hz)}$},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.96,0.94)}, anchor=north east, legend cell align=left, align=left,  font=\footnotesize, draw=white!15!black}
]
\addplot[ybar, bar width=6.829, fill=mycolor1, draw=black, area legend] table[row sep=crcr] {%
1	21.3025142031478\\
2	14.969069981539\\
3	10.7609788355709\\
4	9.76347907422108\\
5	10.3016297706488\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0.514285714285714	0\\
5.48571428571429	0\\
};
\addlegendentry{Indoor}

\addplot[ybar, bar width=6.829, fill=mycolor2, draw=black, area legend] table[row sep=crcr] {%
1	49.6475789519276\\
2	45.0991332363871\\
3	35.2123802329692\\
4	34.2148797084374\\
5	34.7480180175777\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0.514285714285714	0\\
5.48571428571429	0\\
};
\addlegendentry{Outdoor}

\end{axis}
\end{tikzpicture}%

==> figures/sim01.tex <==
\definecolor{ForestGreen}{rgb}{0.1333    0.5451    0.1333}
\definecolor{DarkGoldenrod}{rgb}{0.9333    0.6784    0.0549}
\definecolor{BlueViolet}{rgb}{ 0.6275    0.1255    0.9412}
\definecolor{Firebrick}{rgb}{0.8039    0.1490    0.1490}
\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
  width=2.8in,
  height=1.9in,
  at={(0in,0in)},
scale only axis,
xmin=2,
xmax=14,
xlabel style={font=\color{white!15!black},font=\footnotesize},
xticklabel style = {font=\color{white!15!black},font=\footnotesize},
xlabel={Number of LEO satellites},
ymode=log,
ymin=0.3,
ymax=1000,
yminorticks=true,
ylabel style={font=\color{white!15!black},font=\footnotesize},
yticklabel style = {font=\color{white!15!black},font=\footnotesize},
ylabel={PEB (m)},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(1.02,1.05)}, anchor=south east, legend columns=2, legend cell align=left, align=left, draw=white!15!black, font=\scriptsize}
]
\addplot [color=black, line width=1pt, dashed]
  table[row sep=crcr]{%
2	14276886.6874024\\
4	2632.21201832872\\
6	360.729898754487\\
8	262.387428522945\\
10	182.586577392144\\
12	89.501267916487\\
14	57.4011286771213\\
};
\addlegendentry{Indoor, no RISs }

\addplot [color=black, line width=0.9pt]
  table[row sep=crcr]{%
2	546148.042241049\\
4	100.711281066029\\
6	13.8012450314502\\
8	10.0390094828357\\
10	6.98589257960198\\
12	3.42440976763873\\
14	2.19613693582281\\
};
\addlegendentry{Outdoor, no RISs}

\addplot [color=blue, line width=0.8pt, dashed, mark=*, mark options={solid, blue}, mark size=1.7pt]
  table[row sep=crcr]{%
2	34.2578136783868\\
4	13.6316790878914\\
6	10.529339492242\\
8	9.7025938168044\\
10	6.05172068772251\\
12	5.93589543611359\\
14	5.2824123939792\\
};
\addlegendentry{Indoor, 1 RIS ($\epsilon\!=\!0.995$) }

\addplot [color=blue, line width=0.8pt, mark=*, mark options={solid, blue}, mark size=1.7pt]
  table[row sep=crcr]{%
2	6.12121381887474\\
4	2.95344434161024\\
6	2.31378550430064\\
8	2.16352574031988\\
10	1.16802766145828\\
12	1.09180505353426\\
14	0.903455749452558\\
};
\addlegendentry{Outdoor, 1 RIS ($\epsilon\!=\!0.995$)}

\addplot [color=ForestGreen, line width=0.8pt, dashed, mark=square*, mark options={solid, ForestGreen}, mark size=1.5pt]
  table[row sep=crcr]{%
2	20.0585196134497\\
4	8.10462368980305\\
6	6.13419188664755\\
8	5.59740070023725\\
10	4.08014237479562\\
12	4.03536214407081\\
14	3.58273627291203\\
};
\addlegendentry{Indoor, 1 RIS ($\epsilon\!=\!0.100$) }

\addplot [color=ForestGreen, line width=0.8pt, mark=square*, mark options={solid, ForestGreen}, mark size=1.5pt]
  table[row sep=crcr]{%
2	23.0428720596459\\
4	11.9137928437723\\
6	9.32230930132481\\
8	7.44200078746073\\
10	5.60823773855065\\
12	3.2352500352892\\
14	2.11362937433796\\
};
\addlegendentry{Outdoor, 1 RIS ($\epsilon\!=\!0.100$)}

\addplot [color=red, line width=0.8pt, dashed, mark=triangle*, mark options={solid, red}, mark size=1.7pt]
  table[row sep=crcr]{%
2	8.3295320865432\\
4	3.36805358984643\\
6	2.3334152991651\\
8	2.25503349702613\\
10	1.5057167180047\\
12	1.45191438276551\\
14	1.24395557906563\\
};
\addlegendentry{Indoor, 2 RISs ($\epsilon\!=\!0.100$) }

\addplot [color=red, line width=0.8pt, mark=triangle*, mark options={solid, red}, mark size=1.7pt]
  table[row sep=crcr]{%
2	4.01768765560031\\
4	1.31948123437358\\
6	1.00460395691354\\
8	0.968819425566145\\
10	0.564686453545346\\
12	0.543236473935741\\
14	0.470107823094234\\
};
\addlegendentry{Outdoor, 2 RISs ($\epsilon\!=\!0.995$)}

\end{axis}
\end{tikzpicture}%
